Relational State-Space Model for Stochastic Multi-Object Systems

Real-world dynamical systems often consist of multiple stochastic subsystems that interact with each other. Modeling and forecasting the behavior of such dynamics are generally not easy, due to the inherent hardness in understanding the complicated interactions and evolutions of their constituents. This paper introduces the relational state-space model (R-SSM), a sequential hierarchical latent variable model that makes use of graph neural networks (GNNs) to simulate the joint state transitions of multiple correlated objects. By letting GNNs cooperate with SSM, R-SSM provides a flexible way to incorporate relational information into the modeling of multi-object dynamics. We further suggest augmenting the model with normalizing flows instantiated for vertex-indexed random variables and propose two auxiliary contrastive objectives to facilitate the learning. The utility of R-SSM is empirically evaluated on synthetic and real time-series datasets.

==> data/particles/metrics.tex <==
\begin{tabular}{lrrr}  
\toprule
Steps            & 1                 & 2          & 5  \\
\midrule
Static           & 5.09E-3           & TODO         & TODO       \\
LSTM-indep       & 2.71E-3           & TODO         &  TODO      \\
LSTM-joint       & 1.68E-3           & TODO         &  TODO      \\
NRI              & 1.05E-3           & TODO         &  TODO      \\
\midrule
R-SSM (ours)     & 1.90E-4           & 3.01E-4        &  TODO      \\
\bottomrule
\end{tabular}


==> tex/deprecated.tex <==
Discrete-time state-space models (SSMs), including the widely used
discrete-state hidden Markov model (HMM) and Gaussian linear dynamical system
(LDS), are a class of generative sequential models that serve as workhorses
for dynamical system modeling and sequential data analysis. To model the
sequential data observed from multi-object dynamics with SSMs, the simplest
approach that learns an independent SSM for each individual object is usually
unsatisfactory, because it simply ignores the interactions between objects. A
popular alternative approach is to concatenate the per-object observations
together to construct a high-dimensional time series, based on which a single
SSM is learned in a black-box manner. This approach suffers from two pitfalls.
First, the number of parameters in such models generally scales linearly or
superlinearly with the number of objects, which makes them data-intensive and
limits their scalability. Secondly, black-box models are not always effective
in discovering the interactions between objects, and it is often nontrivial to
inject prior knowledge about interactions into them.

Popular GNN
variants are based on the idea of neural message passing, which simulates how
real-world objects interact in a parameter-efficient way.

\section{Appendix}

\paragraph{Basic Attention Mechanism.}
Given the vertex features $\MH \in \BR^{n \times d}$, we use five parameter
matrices
$\MW_Q \in \BR^{d \times d_k}$,
$\MW_K \in \BR^{d \times d_k}$,
$\MW_V \in \BR^{d \times d_v}$,
$\MW_S \in \BR^{d \times d_v}$ and
$\MW_R \in \BR^{d \times d_v}$
to linearly transform them into queries, keys, values and sender/receiver
attributes, respectively:
$\{\M{Q}, \M{K}, \M{V}, \M{S}, \M{R}\} = \MH \MW_{\{Q,K,V,S,R\}}$.
Below we use the notation $\V{q}_i$ to refer to the $i$-th column vector of
$\V{Q}^{\top}$. For each directed edge $(j, i) \in \CE$, we compute its
compatibility
$c_{j \to i} = \V{q}^{\top}_i \V{k}_j  / \sqrt{d_k} \in \BR$
, i.e., the scaled dot-product similarity between receiver's query and
sender's key. Then for each vertex $i \in \CV$, we turn the compatibilities of
its incoming edges into attention weights:
$
\{a_{p \to i}\}_{p \in \CN^{-}_i} =
\omega \left( \{c_{p \to i}\}_{p \in \CN^{-}_i} \right)
$.
Here $\CN^{-}_i = \left\{p \middle| (p, i) \in \CE\right\}$ is the set of
direct predecessors of vertex $i$, and $\omega(\cdot)$ is an activation
function discussed below. The raw message sent from $j$ to $i$ is computed as
$\V{m}_{j \to i} = \sigma(\V{s}_j \odot \V{r}_i + \V{v}_j)$
, where $\odot$ denotes the Hadamard product and $\sigma(\cdot)$ is an
activation function specified to be $\sigma(x) = x \cdot \text{sigmoid}(x)$ in
this work. Finally each vertex attentively aggregates all raw messages it
received:
$\V{m}_i = \sum_{p \in \CN^{-}_i} a_{p \to i} \V{m}_{p \to i}$,
and the new vertex features are obtained by projecting aggregated messages
$\V{M} = \big[ \V{m}_1, \V{m}_2, \ldots, \V{m}_n \big]^{\top}$
back to a $d$-dimensional space: $\MH' = \V{M}\MW_B$, where $\MW_B \in
\BR^{d_v \times d}$ is another parameter matrix. We write this attention
mechanism as
$\MH' = \text{ATT}(\CG, \MH; \MW_{*}, \omega)$,
where $\MW_* = \MW_{\{Q,K,V,S,R,B\}}$.

In above, to enable the message $\V{m}_{j \to i}$ to depend on both $\Vh_j$
and $\Vh_i$, we have modified the Transformer-style attention by letting
$\V{m}_{j \to i} = \sigma(\V{s}_j \odot \V{r}_i + \V{v}_j)$, where $\V{s}_j$
and $\V{r}_i$ are obtained through two additional transformations $\MW_S$ and
$\MW_R$. Besides, we enable using an activation function other than softmax to
produce the attention weights, e.g., in 3.3 we use uniform weights to ease
the scalable learning procedure. Finally, as pointed in [2][3], in practice it
is often beneficial to allow different types of messages by using multiple
attention heads. Let $M \in \BZ^+$ be a hyperparameter and $\lambda =
\{\MW_*^{(i)} \}_{i=1}^{M}$. We use $M$ separately parameterized attention
heads to compute the new vertex features:
\begin{equation}
\text{MHA}(\CG, \MH; \lambda, \omega) =
\sum_{i=1}^M{
	\text{ATT}(\CG, \MH; \MW_*^{(i)}, \omega)
}
\end{equation}

\paragraph{Attention-based GNNs.} 
An MHA unit only simulates first-order information propogation on the given
graph. In order to capture higher-order interactions, here we further present
how to stack multiple layers of MHA into a GNN block. Let $L \in \BZ^+$ be a
hyperparameter and $\MH^{(0)} = \MH$ be the initial vertex
features. We iteratively compute
$\MH^{(1)}, \MH^{(2)}, \ldots, \MH^{(L)} \eqqcolon \MH'$
as follows:
\[
\M{U}^{(l)} = \text{MHA}\left( \CG, \MH^{(l-1)}; \lambda^{(l)}, \omega \right)
\]
\[
\Vh_i^{(l)} = \text{COMBINE}\left( \Vh_i^{(l-1)}, \V{u}_i^{(l)} \right)
\]
for $i = 1, \ldots, n$, where $\M{U}^{(l)} \in \BR^{n \times d}$ is the matrix
of per-vertex updates at layer $l$, and $\text{COMBINE}$ is a function that
updates $\Vh_i^{(l-1)}$ to $\Vh_i^{(l)}$ conditioning on $\V{u}_i^{(l)}$. In
our case $\text{COMBINE}$ is specified to be a gated recurrent unit (GRU). In
the presentation below we write this GNN construction as $\MH' =
\text{GNN}^{M,L,\omega}(\CG, \MH)$ and treat it as a black box to avoid notational
clutter.

\subsection{Generative Model}

For simplicity, assuming
$\text{RNN}_{\theta}$ is an LSTM and the dimensionality of its cell state is
specified to be $d_h$, then
$\Vh_t^{(i)} \in \BR^{2d_h}$,
$\Vh_1^{(i)} = \V{0}$,
$\tilde{\Vh}_t^{(i)} \in \BR^{d_h}$ and
$\V{c}_t^{(i)} \in \BR^{d_h}$.
Here $\text{FF}_{\theta}$ is a feed-forward layer that combines two LSTM
states and uses $\tanh(\cdot)$ as its activation function, while $f_{\theta}$
and $g_{\theta}$ are tractable distributions parameterized by the output of
‎proper neural networks, e.g., multilayer perceptrons (MLPs). In this work we
take
$
f_{\theta} \left( \cdot \middle| \V{c}_t^{(i)} \right) =
\CN \left(
  \cdot \middle|
  	\bm{\mu}_{\theta}^{\Vz}(\V{c}_t^{(i)}),
  	\bm{\Sigma}_{\theta}^{\Vz}(\V{c}_t^{(i)})
\right)
$
, where $\bm{\mu}_{\theta}$ and $\bm{\Sigma}_{\theta}$ are 2-layer MLPs that
share their first layer. $g_{\theta}$ is specified in a similar way, although
depending on the observations a non-Gaussian distribution may be used. 

\subsection{Scalable Learning}

The learning objective and gradient estimator above involve the full dataset
$\{\Vx_{1:T}^{(i)}\}_{i=1}^N$, resulting in expensive optimization steps if
$N$ or $T$ is large. To scale the proposed model to large datasets, here we
make an assumption that the distribution of the latent state $\Vz_t^{(i)}$
could be well estimated using only vertex $i$'s observations and past states.
This enable us to use a simple structured inference network
$
q'_{\phi}\left( \MZ_{1:T} \middle| \MX_{1:T} \right) =
\prod_{t=1}^T{q'_{\phi}(\MZ_t | \MZ_{<t}, \MX_{\leq t})}
$,
where
$
q'_{\phi}(\MZ_t | \MZ_{<t}, \MX_{\leq t}) =
\prod_{i=1}^N{q'_{\phi}(\Vz_t^{(i)} | \Vz_{<t}^{(i)}, \Vx_{\leq t}^{(i)})}
$
is obtained by replacing $\tilde{\M{B}}_t = \M{B}_t$ into \eqref{eq:2}. Then
we optimize the simpler variational autoencoder (VAE) objective instead:
\begin{equation}
\CL^{\text{VAE}}(\theta, \phi)
= \BE_{q'_{\phi}\left( \MZ_{1:T} \middle| \MX_{1:T} \right)}
\left[
	\log \frac{
		p_{\theta}\left( \MX_{1:T} \middle| \MZ_{1:T} \right)
		p_{\theta}\left( \MZ_{1:T} \right)
	}{
		q'_{\phi}\left( \MZ_{1:T} \middle| \MX_{1:T} \right)
	}
\right]
\end{equation}
The VAE objective is equivalent to $\CL_1^{\text{SMC}}$ if the same proposals
are used. In our case, it factors as a summation over all time steps: 
$
\CL^{\text{VAE}}(\theta, \phi) = \sum_{t=1}^T{
	\BE_{q'_{\phi}\left( \MZ_{<t} \middle| \MX_{<t} \right)}
	\left[ \CF_t \right]
}
$,
where $\CF_t$ is the per-step variational free energy defined as:
\begin{equation} \label{eq:3}
\begin{split}
\CF_t \coloneqq \:
& \BE_{\prod_{i=1}^N{q'_{\phi}(\Vz_t | \Vz_{<t}, \Vx_{\leq t})}}
\left[
	\sum_{i=1}^N{
		\log g_{\theta}\left( \Vx_t^{(i)} \middle| \Vz_t^{(i)} \right)
	}
\right]
\\
& - \sum_{i=1}^N{
	\text{KL}\left(
		q'_{\phi}(\Vz_t^{(i)} | \Vz_{<t}^{(i)}, \Vx_{\leq t}^{(i)} )
		\middle\|
		f_{\theta}( \Vz_t^{(i)} \middle| \V{c}_t^{(i)} )
	\right)
}
\end{split}
\end{equation}
To optimize $\CL^{\text{VAE}}$ in an effective manner, we propose using
graph sampling and truncated backpropagation through time (T-BPTT) to
deal with large $N$ and $T$, respectively.

\paragraph{Graph Sampling.} When there are a large number of vertices, we are
interested in using a sampled subset of them to estimate $\CL^{\text{VAE}}$
(and the reparameterized gradient) at each optimization step. It turns out
that the key challenge here is to estimate $\V{c}_t^{(i)}$ in \eqref{eq:3},
which is produced by the GNN in the generative model and thus depends on the
sampled trajactories of vertex $i$'s $L$-hop neighbors. Here we use
neighborhood sampling [6] to approximate $\V{c}_t^{(i)}$, then estimate the two
terms of \eqref{eq:3} separately. Specifically, at each iteration, we pick a
starting vertex $i$ uniformly at random, and simulate a random walk on the
\emph{reverse} graph with restart probability $1/L$. We donate the set 
of visited vertices as $\CS = \{n_k\}_{k=1}^{|\CS|}$, and let
$\omega(c_{p \to j}) = 1/|\CN_j^- \cap \CS|$.
Then we estimate the VAE objective as:
\[
\CL^{\text{VAE}}(\theta, \phi) \approx \sum_{t=1}^T{
	\BE_{
		\prod_{k=1}^{|\CS|}{
			q'_{\phi}
			\left(\Vz_{<t}^{(n_k)} \middle| \Vx_{<t}^{(n_k)} \right)
		}
	}
	\left[ \tilde{\CF}_t \right]
}
\],
where $\tilde{\CF}_t$ is defined to be:
\begin{equation} \label{eq:4}
\begin{split}
\tilde{\CF}_t \coloneqq \:
& \BE_{
	\prod_{k=1}^{|\CS|}{
		q'_{\phi}
		\left(\Vz_t^{(n_k)} \middle| \Vz_{<t}^{(n_k)}, \Vx_{\leq t}^{(n_k)} \right)
	}
}
\left[
	\frac{N}{|\CS|}
	\sum_{k=1}^{|\CS|}{
		\log g_{\theta}\left( \Vx_t^{(n_k)} \middle| \Vz_t^{(n_k)} \right)
	}
\right]
\\
& - N \cdot
	\text{KL}\left(
		q'_{\phi}(\Vz_t^{(i)} | \Vz_{<t}^{(i)}, \Vx_{\leq t}^{(i)} )
		\middle\|
		f_{\theta}( \Vz_t^{(i)} \middle| \hat{\V{c}}_t^{(i)} )
	\right)
\end{split}
\end{equation}

\paragraph{T-BPTT.} T-BPTT is widely employed to train RNNs on long sequences,
and it can be adapted to our case in a similar way. For large $T$, we
partition $X_{1:T}$ into a sequence of segments
$\{\MX_{t:t+P-1}\}_{t=1}^{\lfloor T/P \rfloor}$, maintain the boundary states
($\MH_{t+P-1}$ and $\tilde{\MB}_{t+P-1}$), and perform truncated
backpropagation on each segment. When $N$ is also large, T-BPTT and graph
sampling can be used together.

\paragraph{Enhancing VSMC with HIS.} The above proposal design 
$
q_{\phi}\left(\MZ_t \middle| \MZ_{<t}, \MX_{\leq t} \right)
= \prod_{i=1}^{N}{
	s_{\phi} \left(\cdot \middle| \V{c}_t^{(i)}, \V{b}_t^{(i)} \right)
}
$
yields a mean-field variational family, which can be not flexible enough to
include members close to the optimal proposal
$p_\theta \left(\MZ_t \middle| \MX_t, \MZ_{<t} \right)$.
Here we follow the idea in the Hamiltonian variational autoencoder (HVAE)
approach and replace the importance sampling step in SMC with HIS targeting
the optimal proposal. Specifically, let $a_{t-1}^k$ be the $k$-th resampled
ancestor index at time $t$, and for notational simplicity let $j = a_{t-1}^k$.
For the ancestral path $\MZ_{<t}^j$, we first propose a sample from the
proposal distribution:
$
\tilde{\MZ}_t^k \sim q_{\phi}\left(
	\cdot \middle| \MZ_{<t}^j, \MX_{\leq t}
\right)
$,
then use target-informed inhomogeneous Hamiltonian dynamics to
deterministically transform $\tilde{\MZ}_t^k$ into some new value $\MZ_t^k$,
and finally compute the importance weight $w_t^k$ for the new particle
$\MZ_{1:t}^k \coloneqq (\MZ_{<t}^j, \MZ_t^k)$ properly. The detailed HIS
procedure is given in the Appendix.


When serving as a sequential generative model, RNN is often augmented with a
parameterized output distribution from some simple distribution family, e.g.,
Gaussian for continuous data. Despite the convenience of tractable likelihood,
it has been observed that such architecture is not sufficient to capture the
complexity of true data distributions \cite{softmax}. 

In VRNN \cite{vrnn}, the variational approximation is structured in the form
of filtering distributions. In SRNN \cite{srnn}, the variational approximation
is designed to mimic smoothing distributions that take the future observations
into account. Z-forcing \cite{zf} introduces an auxiliary cost which forces
the latent variables to reconstruct the summaries of future observations. It
has been observed that such auxiliary task substantially improves the
performance of long-term predictions \cite{zf-rl}.

The state vectors are either coded in a specific form or produced by a learned
perceptual frontend. The whole model is trained with an objective given by
tasks such as future state prediction and scene reconstruction.

We comment that they focus on performing
position estimation and forecasting with partially observed visual
information, whereas we focus on jointly modeling the dynamics of interacting
objects given individual-level observations


Below, we first briefly introduce the VSMC objective and then present the design
of proposal distributions.


It is appealing to augment our model with
a joint meansurement model and a perceptual module to directly learn from
visual data, and we leave this for future work

These models decompose
the scene into a set of objects repesented by state vectors, and model the
interations and dynamics using the neural message passing mechanism. 

Stochastic RNNs can be viewed as special SSMs in which part of the latent
state transition is deterministic and the observation at previous time step
serves as the input of current time step. Compared to autoregressive models,
SSMs that do not depend on observations enable sampling latent state
transitions without generating the intermediate observations, which is an
appealing property for scenarios such as model-based reinforcement learning
when the observation space is high-dimensional. Several recent works  



\paragraph{Correlated Time Series Modeling.} Finally we point out that
correlated time series modeling has been studied extensively in the
spatio-temporal settings \cite{st-book}. Examples include approaches based on
Gaussian process \cite{gp} that model the spatio-temporal correlation using covariance
functions, and statistical dynamic models that model interactions using Markov random fields \cite{tpami-tracking,nested-smc}.


In this section, we empirically evaluate the proposed R-SSM on a variety of
time series modeling tasks to demonstrate its utility. In \ref{ssec:1}, we
illustrate the benefits of relational state space modeling through a toy
example. In \ref{ssec:2}-\ref{ssec:5}, we evaluate the modeling capability and
forecasting performance of R-SSM on several datasets from various domains,
including physics simulations, sports tracking and road traffic.
Overall, we compare R-SSM with following baseline models:
\begin{itemize}
    \item \textbf{RNNs.} We consider two LSTM baselines: (1) LSTM-indep, which
uses an LSTM to autoregressively model the observations of each individual
object and shares the parameters across all objects; and (2) LSTM-joint, which
runs a global LSTM to autoregressively model the concatenated observations of
all objects.
    \item \textbf{Stochastic RNNs.} Stochastic RNNs are generally considered
to have higher modeling capability than vanilla RNNs, thank to the addition of
latent random variables. Our experiments include comparisons with VRNN, SRNN
and Z-forcing.
    \item \textbf{GNNs.} Recent work have shown on simulated and real-world
data that GNN-based forward models support accurate future predictions. We
compare our model with several representative models whose implementations are
publicly available, including Interaction Networks, Graph Networks, DCRNN and
NRI.
\end{itemize}


\subsection{Web Traffic} \label{ssec:5}

Wikimedia Foundation maintains publicly consumable hourly pageview statistics
for every Wikipedia articles, providing a good test bed to examine the
effectiveness of the scalable training procedure. We develop our experiment
based on a preprocessed public dataset[kaggle]. It consists of approximately
145K time series, each of which records the daily view counts of a Wikipedia
article contributed by one type of agents (mobile, desktop, spider, and all).
We select 9K time series that correspond to overall access to all English
articles covered by this dataset. These time series span 983 days from
January 1st, 2015 to September 10th, 2017. We fit and validate our model
using the data of 2015 and 2016, and test the forecasting accuracy on the data
of 2017.

To construct a graph for these articles, we consult the wiki-topcats dataset
and connect two articles if the intersection of their categories is nonempty.
The top-k largest categories are excluded to avoid resulting a dense graph. In
addition, we make use of the Wikipedia Clickstream dataset, another public
dataset maintained by Wikimedia Foundation. It contains (referer, resource)
pairs extracted from the request logs of Wikipedia, i.e., samples of
hyperlinks between Wikipedia articles. We connect two articles if a pair
corresponding to them is found.


    \item \textbf{NYC Traffic Speed}[nyc] made publicly available by NYCDOT.
It provides the average traffic speed of 100 street sections within the five
boroughs of NYC, measured at 5-minute intervals. Each street section is
described as a sequence of latitude/longitude points. To construct the graph,
we connect two street sections if the geodesic distance between the closest
pair of points from them is below a threshold.


Specifically, we use
the R package imputeTS and choose an imputation algorithm which is based on
seasonal decomposition and Kalman smoothing. 


\subsection{Physics Simulations} \label{ssec:2}

In this subsection, we examine our proposed model on simulated physical systems
consisting of interacting particles. Following the settings in \citet{nri}, we
simulate the trajectories of charged particles and
particles connected by springs. In the charged particles model, 10 particles
are bounded inside a 2D box through elastic collisions and interact pairwisely via
electric forces given by Coulomb's law. The springs model is similar, in which
each pair of particles are connected via a spring with a probability 0.5, and
the forces are given by Hooke's law. In each simulation, given randomly
sampled initial locations, the equations of motion are solved using 10,000
steps of leapfrog integration, and the trajectories are generated by
subsampling each 100 steps. We simulate 50K examples for training and 10K
examples for validation and test, respectively.

\begin{table}[h]
  \caption{Multi-step prediction error of different models for particle simulations.}
  \label{particle-table}
  \input{data/particles/metrics}
  \centering
\end{table}


To enable correlated sampling, a possible alternative is a Gaussian Markov random field (GMRF), but it is in general computationally expensive and nontrivial to implement.

. These works differ in the way they wire the
latent variables and the parameterization for the variational distributions.

 and rely on
GNNs to automatically discover the dynamical coordination of players

 (ignoring the ball and the defense
team) 


 and focus
their applications in dynamics modeling here

 to
help infer the state of each object from visual observations


This is expected because seq2seq models explicitly optimize the multistep prediction error.


We find that using another affine layer to add a skip connection from the mean of base Gaussian distribution to the final GNF output helps the optimization.

==> tex/tmp.tex <==
In particular, suppose we have a graph `G = (V, E)`. Following the definition in the beginning, now we additionally assign an initial feature vector `h_i[0]` for each vertex `v_i`. A GNN just takes as input the graph structure `G` and vertex features `H[l] = {h_i[l]: i = 1...N}`, and outputs new vertex features `H[l+1] = {h_i[l+1]: i = 1...N}`, i.e., `GNN(G, H[l]) = H[l+1]`. Here the index `l` can be interprated as _layer_, because a GNN can be stacked on top of itself or other GNNs to update vertex features many times: `GNN(G, GNN(G, GNN(G, H[l]))) = H[l+3]`.

When updating the feature of some vertex `v_i`, GNNs take into consideration the features of other (nearby) vertices. Internally, popular GNN variants implement this by a mechanism called __*message passing*__. Specifically, each vertex sends a message vector to each one of its neighbors, while the content of the message vector may depend on the vertex features of both its sender and receiver. Then each vertex aggregates the messeage vectors that it received, and update its own feature accordingly. [Figure 1](#fig-1) shows a general GNN implementation, which also takes the edge features into consideration.

The message passing mechanism simulates how real-world objects **interact** and **evolve**. Moreover, such modeling capabilities are achieved in a parameter-efficient way. Note that in [Figure 1](#fig-1), only functions `UPDATE`, `AGGREGATE` and `COMBINE` have trainable parameters, so the number of parameters is independent of the number of vertices and edges in the graph. This is an attractive property especially when we are dealing with large graphs that have a lot of vertices. On the other hand, GNNs are also time-efficient, because the time complexity of message passing scales linearly with the number of edges in the graph, which would be a great win if the graph is sparse (i.e., `|E| = o(N^2)`).

Impressed by the unique characteristics and empirical successes of GNNs, we are interested in applying them to time series modeling. In the following subsection we will leave aside GNNs shortly and introduce the _state space models_ first, which use latent random variables to model the latent states of dynamical systems. After that, we show the main idea of this research: incorporating GNNs for modeling the **interactions** and **evolutions** of the latent states of multiple correlated dynamical systems.


\subsection{State Space Models}

**S**tate **S**pace **M**odels are a class of latent variable models designed for modeling dynamical systems. SSMs assume that at each time step `t`, the dynamical system is in some state `z[t]`. Moreover, the state `z[t]` is _**latent**_, means that we cannot directly observe it. Instead, we can only observe some noisy measurements `x[t]` of the latent state: `x[t] ~ g(•|z[t]) <=> x[t] = r(z[t], u[t])`, where `r` is the observation function and `u[t]` is random noise. We call `g` the observation probability density function. In addition, the latent state `z[t]` will _stochastically_ move to a new state `z[t+1]` through a transition probability density function `f`: `z[t+1] ~ f(•|z[t]) <=> z[t+1] = s(z[t], v[t])`, where `s` is the transition function and `v[t]` is random noise. The whole generating process is: starting from some initial latent state `z[1]`, we observe `x[1]`; then the dynamical system move to new latent state `z[2]`, and we observe `x[2]`; and so on. This process can be expressed as the factorized form of joint probability density: `p(x[1:T], z[1:T]) = f(z[1])g(x[1]|z[1]) \product_t_from_2_to_T f(z[t]|z[t-1])g(x[t]|z[t])`. [Figure 2](#fig-2) shows the general graphical model of SSM.

SSMs model the uncertainty in both observations and transitions, making them generally more powerful than autoregressive models. In practice, the observation and tansition functions can be implemented as neural networks, to make the model flexible enough. We thus choose SSM as our basic time series model, and, as introduced in next subsection, enhance its capabilities by letting it cooperate with GNN.

\subsection{Proposal Models}

Suppose we have built a SSM for modeling the obvervation time series of a single vertex, and its parameters are shared across all vertices `{v_i: i = 1...N}`. This is the option [_(2)_](#opt-2) in the [background](#background) section. As we have argued, the problem with this method is that it just assumes the dynamical systems of vertices are evolving independently: `p({z_i[t+1]: i = 1...N}|{z_i[t]: i = 1...N}) = f(z_1[t+1]|z_1[t])...f(z_N[t+1]|z_N[t])`. This simplified assumption is not true in our cases, because the current state of one vertex may affect not only the future state of itself, but also the future state of its neighbors.

As mentioned previously, our main idea is to introduce GNN for modeling the updating process of multiple correlated latent states. Now let us move to the option [_(3)_](#opt-3) and build a single SSM for **all** vertices. Specifically, let `Z[t] = {z_i[t]: i = 1...N}` and `X[t] = {x_i[t]: i = 1...N}`. Note that this is not the concatenating vector approach, because here `Z[t]` and `X[t]` are ordered sets rather than concatenated vectors. The factorized joint density of this SSM is: `p(X[1:T], Z[1:T]) = f(Z[1])g(X[1]|Z[1]) \product_t_from_2_to_T f(Z[t]|Z[t-1])g(X[t]|Z[t])`. Now the remaining problem is how to implement the transition density `f` and observation density `g`. Here we build the transition density with GNNs and leave the observation density simple. More specifically, **multiple layers of GNN** are used for modeling the joint state transitions of all vertices: `Z[t+1] ~ f(•|Z[t]) <=> Z[t+1] = s(GNN_ML(G, Z[t]), V[t])`, where `s` is some custom function and `V[t]` are random noise. Then given the latent state `z_i[t]` of some vertex `v_i` at time step `t`, the observation `x_i[t]` only depends on `z_i[t]`: `x_i[t] ~ g(•|z_i[t]) <=> x_i[t] = r(z_i[t], u_i[t])`, where `r` is the per-vertex observation function and `u_i[t]` is random noise. We call this model **GNN-SSM**, and its graphical model is shown in [Figure 3](#fig-3).

By incorporating GNNs in our generative model, we get efficiencies in number of model parameters, amount of training data, and running time, thus achieve the desired **scalability** and **flexibility**. One question immediately comming along is how to learn the parameters of this model. Latent variable models are generally hard to learn because of the existence of latent random variables. Fortunately, recent advances of **variational inference** methods (e.g., variational autoencoders) make scalable learning of some latent variable models possible. We have developed two methods based on variational inference and more recent **variational sequential Monte Carlo** respectively to learn our proposed model. Currently we are working on experiment design and it is expected that our model will be competitive with state-of-the-arts.

\[
\Vz_0 \sim \mu_{\theta}(\cdot)
\]
\[
\left. \Vz_t \middle| \Vz_{1:t-1} \right. \sim
f_{\theta}\left(\cdot \middle| \Vh_t\right),
\Vh_t = \text{LSTM}_{\theta}(\Vh_{t-1}, \Vz_{t-1})
\]
\[
\left. \Vx_t \middle| \Vz_t \right.
\sim g_{\theta}\left(\cdot \middle| \Vz_t\right)
\]

illustrated

\CN \left(
  \cdot \middle|
  	\bm{\mu}_{\theta}^{\Vz}(\V{c}_t^{(i)}),
  	\bm{\Sigma}_{\theta}^{\Vz}(\V{c}_t^{(i)})
\right)

$
f_{\theta} \left( \cdot \middle| \V{c}_t^{(i)} \right) =
\CN \left(
  \cdot \middle|
  	\bm{\mu}_{\theta}^{\Vz}(\V{c}_t^{(i)}),
  	\bm{\Sigma}_{\theta}^{\Vz}(\V{c}_t^{(i)})
\right)
$

Importance Weight
\[
w_t^k = \frac{
	p_{\theta}\left( \MX_t \middle| \MZ_t^k \right)
	p_{\theta}\left( \MZ_t^k \middle| \MZ_{<t}^{A_t^k} \right)
}{
	q_{\phi}\left( \MZ_t^k \middle| \MZ_{<t}^{A_t^k}, \MX_{1:T} \right)
}
\]

The unbiasedness implies
$
\BE \left[ \hat{p}_{\theta,\phi, K}(\MX_{1:T}) \right]
= p_{\theta}(\MX_{1:T})
$
,

softmax
$
\exp(c_{j \to i}) / \sum_{p \in \CN^{-}_i}{\exp(c_{p \to i})}
$


$\lambda = \{
\V{W}_Q,
\V{W}_K,
\V{W}_V,
\V{W}_S,
\V{W}_R,
\V{W}_M
\}$

\[
\V{Q}=\MH \V{W}_Q\,,\quad
\V{K}=\MH \V{W}_K\,,\quad
\V{V}=\MH \V{W}_V\,,\quad
\V{S}=\MH \V{W}_S\,,\quad
\V{R}=\MH \V{W}_R
\]



\[
\Vh_t^{(i)} =
\text{LSTM}_{\theta}\left( \Vh_{t-1}^{(i)}, \Vz_{t-1}^{(i)} \right)
\]
\[
\V{b}_t^{(i)} =
\text{LSTM}_{\phi}\left( \V{b}_{t+1}^{(i)}, \Vx_t^{(i)} \right)
\]
\[
\big\{ \tilde{\V{b}}_t^{(i)} \big\}_{i=1}^n =
\text{GNN}_{\phi}\left( \CG', \big\{ \V{b}_t^{(i)} \big\}_{i=1}^n \right)
\]
\[
\big\{ \tilde{\Vh}_t^{(i)} \big\}_{i=1}^n =
\text{GNN}_{\phi}\left( \CG, \big\{ \Vh_t^{(i)} \big\}_{i=1}^n \right)
\]
\[
\tilde{\Vz}_t^{(i)} = \text{MLP}\left([\tilde{\Vh}_t^{(i)}, \tilde{\V{b}}_t^{(i)}]\right)
\]
\[
\left. \Vz_t^{(i)} \middle| \big\{ \Vz_{1:t-1}^{(i)} \big\}_{i=1}^n \big\{ \Vz_{1:t-1}^{(i)} \big\}_{i=1}^n \right. \sim
\CN \left(
  \cdot \middle| \text{MLP}_{\phi}^{\V{\mu}_{\Vz}, \V{\sigma}^2_{\Vz}}
  \big( \tilde{\Vz}_t^{(i)} \big)
\right)
\]

[hvae] has proposed to augment
the variational autoencoder (VAE) by using target-informed inhomogeneous
Hamiltonian dynamics to deterministically transform the the samples sampled
from variational posterior approximation, resulting in Hamiltonian VAE (HVAE).

  \sum_{t=1}^T{
    \log \frac{
      p_{\theta}\left( \MX_t \middle| \MZ_t \right)
      p_{\theta}\left( \MZ_t \middle| \MZ_{<t} \right)
    }{
      q'_{\phi}\left( \MZ_t \middle| \MZ_{<t}, \MX_{\leq t} \right)
    }
  }


  Although
simple HMM and LDS are widely used, recent work either incorperate Gaussian
process and neural networks into SSMs to capture complex nonlinear transitions
and/or measurements, or inject latent random variables into vanilla recurrent
neural networks (RNNs) to enhance their modeling capability while in effect
making RNNs become SSMs up to additional inputs. From this perspective,
vanilla RNNs are also SSMs whose state transitions are deterministic
